A Multi-Stage Adaptive Sampling Scheme for Passivity Characterization of Large-Scale Macromodels

This paper proposes a hierarchical adaptive sampling scheme for passivity characterization of large-scale linear lumped macromodels. Here, large-scale is intended both in terms of dynamic order and especially number of input/output ports. Standard passivity characterization approaches based on spectral properties of associated Hamiltonian matrices are either inefficient or non-applicable for large-scale models, due to an excessive computational cost. This paper builds on existing adaptive sampling methods and proposes a hybrid multi-stage algorithm that is able to detect the passivity violations with limited computing resources. Results from extensive testing demonstrate a major reduction in computational requirements with respect to competing approaches.

==> Figures/Testing_Campaign/Summary_20201006.tex <==
%\documentclass[a4paper,10pt]{article}
% Summary of results obtained from data 20201006
%\begin{document}
\begin{table}[t]
\caption{Summary of passivity check results on all benchmark cases. Models are classified as: True Positive (\textbf{TP}), False Positive (\textbf{FP}), False Negative (\textbf{FN}), see text}
\label{table: Summary_20201006}
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\# Tests & Passive & TP & FP & FN & Passive but FN \\
\hline
447 & 179 & 446 & 0 & 1 & 1\\
\hline
\end{tabular}
%\caption{Summary of passivity check results on all available test-cases. Models are classified as: True Positive (\textbf{TP}), if both an adaptive sampling and an Hamiltonian based passivity check (using Matlab) produced the same outcome (passive or not); False Positive (\textbf{FP}), if the adaptive sampling approach identified a passive model while the Hamiltonian check did not; False Negative (\textbf{FN}), if the Hamiltonian classified a model as passive while the adaptive sampling did not; \textbf{Passive but FN} indicates models that are really non-passive even if the Hamiltonian check did not find any passivity violation. Code errors are reported in the last column.}
\end{table}
%\end{document}


==> PDNMSO.tex <==
\begin{algorithm}
	\SetKw{and}{and} 
	\SetKw{or}{or}
	\SetKwInput{Ctrl}{Control Parameters}
    \caption{Passivity-Driven NMSO}\label{algo: PD-NMSO}
    \KwIn{Target function $\ssr$ and passivity treshold $\gamma$}
    \Ctrl{$\Ch$; $\delta_x$; $\delta_y$; $\delta_p$; Evaluation budged vector $\vet{n}^e = [n_0^e, \dots , n_{max}^e]$}
    Initialization: $h \leftarrow 0$, $\mathcal{E} \leftarrow \emptyset$, $\mu \leftarrow 0$, maximum $\ssr_{m} = 0$, $c = 0$, evaluation budget $n_\mu = n^e_c$ \;
    Evaluate tree root $\ssr(\omw_{0, 0})$\;
    Set initial refinement $h_0 = h+1$\;
    Expand children $\ssr(\omw_{h_o, i})$ \tcp*{Initial sampling}
    \While{$n_\mu > 0$}{
    	$\mu \leftarrow \mu+1$ \tcp*{Increase iter counter}
    	%$h \leftarrow h+1$ \tcp*{Increase tree level}
    	\uIf{$\exists \omw_{h,i} \in\mathcal{C}_{\mu}$}{
    		$\omw_{h,\ibest} = \arg\max_{(h,i)} \{\ssr(\omw_{h,i}):\, \omw_{h,i}\in\mathcal{C}_{\mu}\}$
    	}
    	\uElseIf{$\exists \omw_{h+1,i} \in\mathcal{E}_{\mu}$}{
    		\textbf{continue} \tcp*{Max depth not reached}
    	}
    	\Else{
    		\Return \tcp*{Budget not completed}
    	}
    	$j_{max} = M(\ibest+1)-1$\;
    	\If{$ M > n_\mu$}{
    	\tcp*{do not exceed budget}
    	%%%%%$M \leftarrow n_\mu$ \tcp*{Particular case}
    	$j_{max} \leftarrow j_{max} - (M-n_\mu)$
    	}
     	\Begin(Expansion process){ 
     	    %$\{\omw_{h+1,j},\;j=M\ibest,\dots,M(\ibest+1)-1\}$\;
     	    $\{\omw_{h+1,j},\;j=M\ibest,\dots,j_{max}\}$\;
     		Evaluate children $\ssr(\omw_{h+1,j})$\;
     		%Find  $\ssr_\mu = \max_{(h+1, j)} \{\ssr(\omw_{h+1,j}) ,\;j=M\ibest,\dots,M(\ibest+1)-1\}$\;
     		Find  $\ssr_\mu = \max_{(h+1, j)} \{\ssr(\omw_{h+1,j}) ,\;j=M\ibest,\dots,j_{max}\}$\;
     		$n_\mu \leftarrow n_\mu - M$ \tcp*{Update budget}
     		}
%    	Expansion process: $\{\omw_{h+1,j},\;j=M\ibest,\dots,M(\ibest+1)-1\}$\;
%    	Evaluate children $\ssr(\omw_{h+1,j})$\;
%    	$n_\mu \leftarrow n_\mu - M$ \tcp*{Update budget}
%    	Find  $\ssr_\mu = \max_{(h+1, i)} \{\ssr(\omw_{h+1,j}) ,\;j=M\ibest,\dots,M(\ibest+1)-1\}$\;
    	\If{$\ssr_\mu>\ssr_m$}{
    		$\ssr_m = \ssr_\mu $}
    	\If{$\ssr_\mu<\delta$ \and \eqref{eq: critical} \and \eqref{eq: critical_rel_distance} }{
    		\If{$n_\mu \leq 0$}{\tcp*{Boost}
    			%%%%$M \leftarrow default$ \tcp*{Particular case}
	    		$c \leftarrow c + 1$\;
	    		$n_\mu \leftarrow n^e_c - n^e_{c-1} $\;
	    		$\varepsilon \leftarrow d \cdot \varepsilon$ }
    	}
    	\uIf{\eqref{eq: restart} \or \eqref{eq: restart_last}}{
    		$\mathcal{B}_{\mu+1} = \mathcal{B}_\mu \cup \{\omw_{h+1,j},\;j=M\ibest,\dots,j_{max}\} $\;
    		$\varepsilon \leftarrow default$\;
    		$h \leftarrow 0$}
    	\Else{
    	%$\mathcal{C}_{\mu+1} = \mathcal{C}_\mu \cup \{\omw_{h+1,j},\;j=M\ibest,\dots,M(\ibest+1)-1\} $\;
    	$\mathcal{C}_{\mu+1} = \mathcal{C}_\mu \cup \{\omw_{h+1,j},\;j=M\ibest,\dots,j_{max}\} $\;
    	{\color{red}$h \leftarrow h+1$ \tcp*{Increase tree level}}
    	}
    }
    \KwOut{Maximum of the target function $\ssr_m$, $\mathcal{E}$}
\end{algorithm}
